Microlensing events indicate that super-Earth exoplanets are common in Jupiter-like orbits

Exoplanets classified as super-Earths are commonly observed on short period orbits, close to their host stars, but their abundance on wider orbits is poorly constrained. Gravitational microlensing is sensitive to exoplanets on wide orbits. We observed the microlensing event OGLE-2016-BLG-0007, which indicates an exoplanet with a planet-to-star mass ratio roughly double the Earth-Sun mass-ratio, on an orbit longer than Saturn's. We combine this event with a larger sample from a microlensing survey to determine the distribution of mass ratios for planets on wide orbits. We infer there are $\sim 0.35$ super-Earth planets per star on Jupiter-like orbits. The observations are most consistent with a bimodal distribution, with separate peaks for super-Earths and gas giants. We suggest that this reflects differences in their formation processes.

==> backup.tex <==
\begin{thebibliography}{100}

% Main Text 
\bibitem{Borucki11}
W.~J. {Borucki}, {\it et~al.\/}, {Characteristics of Kepler Planetary
  Candidates Based on the First Data Set}. {\it Astrophysical Journal\/} {\bf 728}, 117 (2011).

\bibitem{Mayor11}
M.~{Mayor}, {\it et~al.\/}, {The HARPS search for southern extra-solar planets
  XXXIV. Occurrence, mass distribution and orbital properties of super-Earths
  and Neptune-mass planets}. {\it arXiv e-prints\/} p. arXiv:1109.2497 (2011).

\bibitem{Wittenmyer11}
R.~A. {Wittenmyer}, {\it et~al.\/}, {The Frequency of Low-mass Exoplanets. III.
  Toward {\ensuremath{\eta}}$_{{\ensuremath{\oplus}}}$ at Short Periods}. {\it
  Astrophysical Journal\/} {\bf 738}, 81 (2011).

\bibitem{Bonfils13}
X.~{Bonfils}, {\it et~al.\/}, {The HARPS search for southern extra-solar
  planets. XXXI. The M-dwarf sample}. {\it Astronomy and Astrophysics\/} {\bf 549}, A109 (2013).

\bibitem{Suzuki16}
D.~{Suzuki}, {\it et~al.\/}, {The Exoplanet Mass-ratio Function from the MOA-II
  Survey: Discovery of a Break and Likely Peak at a Neptune Mass}. {\it Astrophysical Journal\/}
  {\bf 833}, 145 (2016).

\bibitem{Shvartzvald16}
Y.~{Shvartzvald}, {\it et~al.\/}, {The frequency of snowline-region planets
  from four years of OGLE-MOA-Wise second-generation microlensing}. {\it
  Mon. Not. R. Astron. Soc.\/} {\bf 457}, 4089 (2016).

\bibitem{Poleski21}
R.~{Poleski}, {\it et~al.\/}, {Wide-Orbit Exoplanets are Common. Analysis of
  Nearly 20 Years of OGLE Microlensing Survey Data}. {\it Acta Astronomica\/} {\bf 71}, 1
  (2021). 

\bibitem{Kim16_KMTNet}
S.-L. {Kim}, {\it et~al.\/}, {KMTNET: A Network of 1.6 m Wide-Field Optical
  Telescopes Installed at Three Southern Observatories}. {\it Journal of Korean
  Astronomical Society\/} {\bf 49}, 37 (2016).

\bibitem{KimKim18_EF}
D.~J. {Kim}, {\it et~al.\/}, {Korea Microlensing Telescope Network Microlensing
  Events from 2015: Event-finding Algorithm, Vetting, and Photometry}. {\it
  Astronomical Journal\/} {\bf 155}, 76 (2018).
  
 \bibitem{Kim18EF}
H.-W. {Kim}, {\it et~al.\/}, {The KMTNet 2016 Data Release}. {\it ArXiv
  e-prints\/}  (2018).

\bibitem{Kim18_AF}
H.-W. {Kim}, {\it et~al.\/}, {The Korea Microlensing Telescope Network (KMTNet)
  Alert Algorithm and Alert System}. {\it arXiv e-prints\/} p. arXiv:1806.07545
  (2018).

\bibitem{Zang21AF1}
W.~{Zang}, {\it et~al.\/}, {Systematic KMTNet Planetary Anomaly Search. I.
  OGLE-2019-BLG-1053Lb, a Buried Terrestrial Planet}. {\it Astronomical Journal\/} {\bf 162},
  163 (2021).
  

\bibitem{Zang22AF4}
W.~{Zang}, {\it et~al.\/}, {Systematic KMTNet planetary anomaly search. IV.
  Complete sample of 2019 prime-field}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 515}, 928 (2022).

\bibitem{Udalski1994}
A.~{Udalski}, {\it et~al.\/}, {The Optical Gravitational Lensing Experiment.
  The Early Warning System: Real Time Microlensing}. {\it Acta Astronomica\/} {\bf 44},
  227 (1994).
  
\bibitem{Udalski2003}
A.~{Udalski}, {The Optical Gravitational Lensing Experiment. Real Time Data
  Analysis Systems in the OGLE-III Survey}. {\it Acta Astronomica\/} {\bf 53}, 291
  (2003).

\bibitem{MatMeth}
Materials and methods are available as supplementary materials.

\bibitem{Gaudi98}
B.~S. {Gaudi}, {Distinguishing Between Binary-Source and Planetary Microlensing
  Perturbations}. {\it Astrophysical Journal\/} {\bf 506}, 533 (1998).

\bibitem{Burn21_BERN4}
R.~{Burn}, {\it et~al.\/}, {The New Generation Planetary Population Synthesis
  (NGPPS). IV. Planetary systems around low-mass stars}. {\it Astronomy and Astrophysics\/} {\bf
  656}, A72 (2021).
  
\bibitem{StarovoitRodin17}
E.~D. {Starovoit}, A.~E. {Rodin}, {On the existence of planets around the
  pulsar PSR B0329+54}. {\it Astronomy Reports\/} {\bf 61}, 948 (2017).

\bibitem{PatrunoKama17}
A.~{Patruno}, M.~{Kama}, {Neutron star planets: Atmospheric processes and
  irradiation}.  {\it Astronomy and Astrophysics\/} {\bf 608}, A147 (2017).
  
\bibitem{Gould22AF5}
A.~{Gould}, {\it et~al.\/}, {Systematic KMTNet planetary anomaly search. V.
  Complete sample of 2018 prime-field}. {\it Astronomy and Astrophysics\/} {\bf 664}, A13 (2022).

\bibitem{Jung22AF6}
Y.~K. {Jung}, {\it et~al.\/}, {Systematic KMTNet Planetary Anomaly Search. VI.
  Complete Sample of 2018 Sub-prime-field Planets}. {\it Astronomical Journal\/} {\bf 164}, 262
  (2022).

\bibitem{Jung23AF8}
Y.~K. {Jung}, {\it et~al.\/}, {Systematic KMTNet Planetary Anomaly Search.
  VIII. Complete Sample of 2019 Subprime Field Planets}. {\it Astronomical Journal\/} {\bf 165},
  226 (2023).

\bibitem{Hwang22AF2}
K.-H. {Hwang}, {\it et~al.\/}, {Systematic KMTNet Planetary Anomaly Search. II.
  Six New q $<$ 2 {\texttimes} 10$^{-4}$ Mass-ratio Planets}. {\it Astronomical Journal\/} {\bf
  163}, 43 (2022).

\bibitem{Zang23AF7}
W.~{Zang}, {\it et~al.\/}, {Systematic KMTNet Planetary Anomaly Search. VII.
  Complete Sample of q $<$ 10$^{-4}$ Planets from the First 4 yr Survey}. {\it
  Astronomical Journal\/} {\bf 165}, 103 (2023).

\bibitem{Pollack96}
J.~B. {Pollack}, {\it et~al.\/}, {Formation of the Giant Planets by Concurrent
  Accretion of Solids and Gas}. {\it Icarus\/} {\bf 124}, 62 (1996).

\bibitem{PapaloizouNelson05}
J.~C.~B. {Papaloizou}, R.~P. {Nelson}, {Models of accreting gas giant
  protoplanets in protostellar disks}. {\it Astronomy and Astrophysics\/} {\bf 433}, 247 (2005).

\bibitem{Coleman17}
G.~A.~L. {Coleman}, J.~C.~B. {Papaloizou}, R.~P. {Nelson}, {In situ accretion
  of gaseous envelopes on to planetary cores embedded in evolving
  protoplanetary discs}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 470}, 3206 (2017).

\bibitem{Boss97}
A.~P. {Boss}, {Giant planet formation by gravitational instability.} {\it
  Science\/} {\bf 276}, 1836 (1997).

\bibitem{Udalski18}
A.~{Udalski}, {\it et~al.\/}, {OGLE-2017-BLG-1434Lb: Eighth
  $q<1\times10^{-4}$ Mass-Ratio Microlens Planet Confirms Turnover in
  Planet Mass-Ratio Function}. {\it Acta Astronomica\/} {\bf 68}, 1 (2018).

\bibitem{Jung19_0165}
Y.~K. {Jung}, {\it et~al.\/}, {KMT-2017-BLG-0165Lb: A Super-Neptune-mass Planet
  Orbiting a Sun-like Host Star}. {\it Astronomical Journal\/} {\bf 157}, 72 (2019).

\bibitem{Gould10}
A.~{Gould}, {\it et~al.\/}, {Frequency of Solar-like Systems and of Ice and Gas
  Giants Beyond the Snow Line from High-magnification Microlensing Events in
  2005-2008}. {\it Astrophysical Journal\/} {\bf 720}, 1073 (2010).

\bibitem{ClantonGaudi16}
C.~{Clanton}, B.~S. {Gaudi}, {Synthesizing Exoplanet Demographics: A Single
  Population of Long-period Planetary Companions to M Dwarfs Consistent with
  Microlensing, Radial Velocity, and Direct Imaging Surveys}. {\it Astrophysical Journal\/} {\bf
  819}, 125 (2016).

\bibitem{Suzuki18}
D.~{Suzuki}, {\it et~al.\/}, {Microlensing Results Challenge the Core Accretion
  Runaway Growth Scenario for Gas Giants}. {\it Astrophysical Journal\/} {\bf 869}, L34 (2018).

\bibitem{GoldreichTremaine80}
P.~{Goldreich}, S.~{Tremaine}, {Disk-satellite interactions.} {\it Astrophysical Journal\/} {\bf
  241}, 425 (1980).

\bibitem{LinPapaloizou86}
D.~N.~C. {Lin}, J.~{Papaloizou}, {On the Tidal Interaction between Protoplanets
  and the Protoplanetary Disk. III. Orbital Migration of Protoplanets}. {\it
  Astrophysical Journal\/} {\bf 309}, 846 (1986).

\bibitem{IdaLin04}
S.~{Ida}, D.~N.~C. {Lin}, {Toward a Deterministic Model of Planetary Formation.
  I. A Desert in the Mass and Semimajor Axis Distributions of Extrasolar
  Planets}. {\it Astrophysical Journal\/} {\bf 604}, 388 (2004).

\bibitem{Ida05}
S.~{Ida}, D.~N.~C. {Lin}, {Toward a Deterministic Model of Planetary Formation.
  III. Mass Distribution of Short-Period Planets around Stars of Various
  Masses}. {\it Astrophysical Journal\/} {\bf 626}, 1045 (2005).

\bibitem{Alibert05}
Y.~{Alibert}, C.~{Mordasini}, W.~{Benz}, C.~{Winisdoerffer}, {Models of giant
  planet formation with migration and disc evolution}. {\it Astronomy and Astrophysics\/} {\bf 434},
  343 (2005).

\bibitem{Mordasini12}
C.~{Mordasini}, Y.~{Alibert}, H.~{Klahr}, T.~{Henning}, {Characterization of
  exoplanets from their formation. I. Models of combined planet formation and
  evolution}. {\it Astronomy and Astrophysics\/} {\bf 547}, A111 (2012).

\bibitem{Boss23}
A.~P. {Boss}, S.~{Kanodia}, {Forming Gas Giants Around a Range of Protostellar
  M-dwarfs by Gas Disk Gravitational Instability}. {\it Astrophysical Journal\/} {\bf 956}, 4 (2023).

%%% Main Figure Captions %%%
 \bibitem{NEA}
R.~L. {Akeson}, {\it et~al.\/}, {The NASA Exoplanet Archive: Data and Tools for
  Exoplanet Research}. {\it Publ. Astron. Soc. Pac.\/}  {\bf 125}, 989 (2013).
  
%%% Main Table captions %%%

%%% Acknowledgments %%%
\bibitem{10.26093/cds/vizier}
{The VizieR database of astronomical catalogues}
doi:10.26093/cds/vizier

\bibitem{vizier2000}
F. {Ochsenbein}, P. {Bauer},  and J. {Marcout},
{The VizieR database of astronomical catalogues}. {\it Astronomy and Astrophysics, Supplement\/} {\bf 143}, 23 (2000).
%%% Data Release Statement %%%

\bibitem{Data}
Microlensing events indicate that super-Earth exoplanets are common in Jupiter-like orbits, Dryad (2024) doi:10.5061/dryad.ksn02v7cg
% [temporary link:  https://datadryad.org/stash/share/af155Huhv4dUI6CcuZGpS7URN5xNJTfE7bqdNejSGtI]

\bibitem{OGLEIII}
M.~K. {Szyma{\'n}ski}, {\it et~al.\/}, {The Optical Gravitational Lensing
  Experiment. OGLE-III Photometric Maps of the Galactic Bulge Fields}. {\it
  Acta Astronomica\/} {\bf 61}, 83 (2011).

\bibitem{Claret11}
A.~{Claret}, S.~{Bloemen}, {Gravity and limb-darkening coefficients for the
  Kepler, CoRoT, Spitzer, uvby, UBVRIJHK, and Sloan photometric systems}. {\it Astronomy and Astrophysics\/} {\bf 529}, A75 (2011).


%%% Supplementary Materials text %%%

\bibitem{Bond01}
I.~A. {Bond}, {\it et~al.\/}, {Real-time difference imaging analysis of MOA
  Galactic bulge observations during 2000}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 327}, 868
  (2001).

\bibitem{Udalski15_OGLEIV}
A.~{Udalski}, M.~K. {Szyma{\'n}ski}, G.~{Szyma{\'n}ski}, {OGLE-IV: Fourth Phase
  of the Optical Gravitational Lensing Experiment}. {\it Acta Astronomica\/} {\bf 65}, 1
  (2015).

\bibitem{Sako2008}
T.~{Sako}, {\it et~al.\/}, {MOA-cam3: a wide-field mosaic CCD camera for a
  gravitational microlensing survey in New Zealand}. {\it Experimental
  Astronomy\/} {\bf 22}, 51 (2008).

\bibitem{Tomaney1996}
A.~B. {Tomaney}, A.~P.~S. {Crotts}, {Expanding the Realm of Microlensing
  Surveys with Difference Image Photometry}. {\it Astronomical Journal\/} {\bf 112}, 2872
  (1996).

\bibitem{Alard1998}
C.~{Alard}, R.~H. {Lupton}, {A Method for Optimal Image Subtraction}. {\it
  Astrophysical Journal\/} {\bf 503}, 325 (1998).

\bibitem{Wozniak2000}
P.~R. {Wozniak}, {Difference Image Analysis of the OGLE-II Bulge Data. I. The
  Method}. {\it Acta Astronomica\/} {\bf 50}, 421 (2000).

\bibitem{Albrow09}
M.~D. {Albrow}, {\it et~al.\/}, {Difference imaging photometry of blended
  gravitational microlensing events with a numerical kernel}. {\it Mon. Not. R. Astron. Soc.\/}
  {\bf 397}, 2099 (2009).

\bibitem{Yang23_pySIS}
H.~{Yang}, {\it et~al.\/}, {Systematic reanalysis of KMTNet microlensing
  events, paper I: Updates of the photometry pipeline and a new planet
  candidate}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 528}, 11 (2024).

\bibitem{pyDIA}
M.~D. {Albrow}, {Michaeldalbrow/Pydia: Initial Release On Github.} 
{\it Zenodo} doi: 10.5281/zenodo.268049. (2017).


\bibitem{MulensModel}
R.~{Poleski}, J.~C. {Yee}, {Modeling microlensing events with MulensModel}.
  {\it Astronomy and Computing\/} {\bf 26}, 35 (2019).
  
\bibitem{Ryu22_MP1}
Y.-H. {Ryu}, {\it et~al.\/}, {Mass Production of 2021 KMTNet Microlensing
  Planets. I}. {\it Astronomical Journal\/} {\bf 164}, 180 (2022).

\bibitem{GouldLoeb92}
A.~{Gould}, A.~{Loeb}, {Discovering planetary systems through gravitational
  microlenses}. {\it Astrophysical Journal\/} {\bf 396}, 104 (1992).

\bibitem{Han06}
C.~{Han}, {Properties of Planetary Caustics in Gravitational Microlensing}.
  {\it Astrophysical Journal\/} {\bf 638}, 1080 (2006).

\bibitem{WittMao95}
H.~J. {Witt}, S.~{Mao}, {On the Minimum Magnification Between Caustic Crossings
  for Microlensing by Binary and Multiple Stars}. {\it Astrophysical Journal\/} {\bf 447}, L105
  (1995).
  
\bibitem{MaoPaczynski91}
S.~{Mao}, B.~{Paczynski}, {Gravitational microlensing by double stars and
  planetary systems}. {\it Astrophysical Journal\/} {\bf 374}, L37 (1991).
  
\bibitem{GouldGaucherel97}
A.~{Gould}, C.~{Gaucherel}, {Stokes's Theorem Applied to Microlensing of Finite
  Sources}. {\it Astrophysical Journal\/} {\bf 477}, 580 (1997).
  
\bibitem{emcee}
D.~{Foreman-Mackey}, D.~W. {Hogg}, D.~{Lang}, J.~{Goodman}, {emcee: The MCMC
  Hammer}. {\it Publ. Astron. Soc. Pac.\/} {\bf 125}, 306 (2013).

\bibitem{scipy}
P.~Virtanen, {\it et~al.\/}, {{SciPy} 1.0: Fundamental Algorithms for
  Scientific Computing in Python}. {\it Nature Methods\/} {\bf 17}, 261 (2020).

\bibitem{Bozza2010}
V.~{Bozza}, {Microlensing with an advanced contour integration algorithm:
  Green's theorem to third order, error control, optimal sampling and limb
  darkening}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 408}, 2188 (2010).

\bibitem{Bozza2018}
V.~{Bozza}, {\it et~al.\/}, {VBBINARYLENSING: a public package for microlensing
  light-curve computation}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 479}, 5157 (2018).

\bibitem{Gould1992}
A.~{Gould}, {Extending the MACHO search to about 10 exp 6 solar masses}. {\it
  Astrophysical Journal\/} {\bf 392}, 442 (1992).

\bibitem{Gould2000}
A.~{Gould}, {A Natural Formalism for Microlensing}. {\it Astrophysical Journal\/} {\bf 542}, 785
  (2000).

\bibitem{Gouldpies2004}
A.~{Gould}, {Resolution of the MACHO-LMC-5 Puzzle: The Jerk-Parallax Microlens
  Degeneracy}. {\it Astrophysical Journal\/} {\bf 606}, 319 (2004).

\bibitem{MB09387}
V.~{Batista}, {\it et~al.\/}, {MOA-2009-BLG-387Lb: a massive planet orbiting an
  M dwarf}. {\it Astronomy and Astrophysics\/} {\bf 529}, A102 (2011).

\bibitem{OB09020}
J.~{Skowron}, {\it et~al.\/}, {Binary Microlensing Event OGLE-2009-BLG-020
  Gives Verifiable Mass, Distance, and Orbit Predictions}. {\it Astrophysical Journal\/} {\bf
  738}, 87 (2011).

\bibitem{MB12486}
K.-H. {Hwang}, {\it et~al.\/}, {Interpretation of a Short-term Anomaly in the
  Gravitational Microlensing Event MOA-2012-BLG-486}. {\it Astrophysical Journal\/} {\bf 778},
  55 (2013).

\bibitem{MASADA}
A.~{Gould}, {MASADA: From Microlensing Planet Mass-Ratio Function to Planet
  Mass Function}. {\it arXiv e-prints\/} p. arXiv:2209.12501 (2022).

\bibitem{Nataf13}
{Nataf}, D.~M., {Gould}, A., {Fouqu{\'e}}, P., {et~al.},  {Reddening and Extinction toward the Galactic Bulge from OGLE-III: The Inner Milky Way's R$_{V}$ \raisebox{-0.5ex}\textasciitilde 2.5 Extinction Curve} {\it Astrophysical Journal\/} {\bf 769}, 88 (2013).

\bibitem{GaiaDR3}
{Gaia Collaboration}, {\it et~al.\/}, {Gaia Data Release 3. Summary of the
  contents and survey properties}. {\it Astronomy and Astrophysics\/} {\bf 674}, A1 (2023).

\bibitem{Clarke19}
J.~P. {Clarke}, {\it et~al.\/}, {The Milky Way bar/bulge in proper motions: a
  3D view from VIRAC and Gaia}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 489}, 3519 (2019).

\bibitem{Yoo04_CMDMethod}
J.~{Yoo}, {\it et~al.\/}, {OGLE-2003-BLG-262: Finite-Source Effects from a
  Point-Mass Lens}. {\it Astrophysical Journal\/} {\bf 603}, 139 (2004).

\bibitem{Bensby2013}
T.~{Bensby}, {\it et~al.\/}, {Chemical evolution of the Galactic bulge as
  traced by microlensed dwarf and subgiant stars. V. Evidence for a wide age
  distribution and a complex MDF}. {\it Astronomy and Astrophysics\/} {\bf 549}, A147 (2013).

\bibitem{Nataf2013}
D.~M. {Nataf}, {\it et~al.\/}, {Reddening and Extinction toward the Galactic
  Bulge from OGLE-III: The Inner Milky Way's R$_{V}$ \~{} 2.5 Extinction
  Curve}. {\it Astrophysical Journal\/} {\bf 769}, 88 (2013).

\bibitem{Bessell1988}
M.~S. {Bessell}, J.~M. {Brett}, {JHKLM photometry - Standard systems,
  passbands, and intrinsic colors}. {\it Publ. Astron. Soc. Pac.\/} {\bf 100}, 1134 (1988).

\bibitem{Adams2018}
A.~D. {Adams}, T.~S. {Boyajian}, K.~{von Braun}, {Predicting stellar angular
  diameters from V, I$_{C}$, H and K photometry}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 473},
  3608 (2018).

\bibitem{Houdashelt2000}
M.~L. {Houdashelt}, R.~A. {Bell}, A.~V. {Sweigart}, {Improved Color-Temperature
  Relations and Bolometric Corrections for Cool Stars}. {\it Astronomical Journal\/} {\bf 119},
  1448 (2000).

\bibitem{Claret2011}
A.~{Claret}, S.~{Bloemen}, {Gravity and limb-darkening coefficients for the
  Kepler, CoRoT, Spitzer, uvby, UBVRIJHK, and Sloan photometric systems}. {\it
  Astronomy and Astrophysics\/} {\bf 529}, A75 (2011).

\bibitem{OB180532}
Y.-H. {Ryu}, {\it et~al.\/}, {OGLE-2018-BLG-0532Lb: Cold Neptune with Possible
  Jovian Sibling}. {\it Astronomical Journal\/} {\bf 160}, 183 (2020).

\bibitem{KB181025}
C.~{Han}, {\it et~al.\/}, {KMT-2018-BLG-1025Lb: microlensing super-Earth planet
  orbiting a low-mass star}. {\it Astronomy and Astrophysics\/} {\bf 649}, A90 (2021).

\bibitem{KB191953}
C.~{Han}, {\it et~al.\/}, {One Planet or Two Planets? The Ultra-sensitive
  Extreme-magnification Microlensing Event KMT-2019-BLG-1953}. {\it Astronomical Journal\/} {\bf
  160}, 17 (2020).

\bibitem{OB181700}
C.~{Han}, {\it et~al.\/}, {OGLE-2018-BLG-1700L: Microlensing Planet in Binary
  Stellar System}. {\it Astronomical Journal\/} {\bf 159}, 48 (2020).

\bibitem{KB191715}
C.~{Han}, {\it et~al.\/}, {KMT-2019-BLG-1715: Planetary Microlensing Event with
  Three Lens Masses and Two Source Stars}. {\it Astronomical Journal\/} {\bf 161}, 270 (2021).

\bibitem{OB191470}
R.~{Kuang}, {\it et~al.\/}, {OGLE-2019-BLG-1470LABc: Another microlensing giant
  planet in a binary system?} {\it Mon. Not. R. Astron. Soc.\/} {\bf 516}, 1704 (2022).

\bibitem{Hwang18_0212}
K.~H. {Hwang}, {\it et~al.\/}, {KMT-2016-BLG-0212: First KMTNet-Only Discovery
  of a Substellar Companion}. {\it Journal of Korean Astronomical Society\/}
  {\bf 51}, 197 (2018).
  
\bibitem{Shin23_AF9}
I.-G. {Shin}, {\it et~al.\/}, {Systematic KMTNet Planetary Anomaly Search. IX.
  Complete Sample of 2016 Prime-Field Planets}. {\it Astronomical Journal\/} {\bf 166},104 (2023).

\bibitem{Gaudi1998}
B.~S. {Gaudi}, {Distinguig Between Binary-Source and Planetary Microlensing
  Perturbations}. {\it Astrophysical Journal\/} {\bf 506}, 533 (1998).

\bibitem{KB181988}
C.~{Han}, {\it et~al.\/}, {KMT-2018-BLG-1988Lb: Microlensing super-Earth
  orbiting a low-mass disk dwarf}. {\it Astronomy and Astrophysics\/} {\bf 658}, A62 (2022).

\bibitem{OB171691}
C.~{Han}, {\it et~al.\/}, {Four sub-Jovian-mass planets detected by
  high-cadence microlensing surveys}. {\it Astronomy and Astrophysics\/} {\bf 664}, A33 (2022).

\bibitem{OB180596}
Y.~K. {Jung}, {\it et~al.\/}, {Spitzer Parallax of OGLE-2018-BLG-0596: A
  Low-mass-ratio Planet around an M Dwarf}. {\it Astronomical Journal\/} {\bf 158}, 28 (2019).

\bibitem{Gaudi02}
B.~S. {Gaudi}, {\it et~al.\/}, {Microlensing Constraints on the Frequency of
  Jupiter-Mass Companions: Analysis of 5 Years of PLANET Photometry}. {\it
  Astrophysical Journal\/} {\bf 566}, 463 (2002).
  
\bibitem{Spada17}
F.~{Spada}, P.~{Demarque}, Y.~C. {Kim}, T.~S. {Boyajian}, J.~M. {Brewer}, {The
  Yale-Potsdam Stellar Isochrones}.  {\it Astrophysical Journal\/} {\bf 838}, 161 (2017).
  
 \bibitem{Jung21}
Y.~K. {Jung}, {\it et~al.\/}, {OGLE-2018-BLG-0567Lb and OGLE-2018-BLG-0962Lb:
  Two Microlensing Planets through the Planetary-caustic Channel}. {\it Astronomical Journal\/}
  {\bf 161}, 293 (2021).


\bibitem{Alcock1996}
C.~{Alcock}, {\it et~al.\/}, {The MACHO Project First-Year Large Magellanic
  Cloud Results: The Microlensing Rate and the Nature of the Galactic Dark
  Halo}. {\it Astrophysical Journal\/} {\bf 461}, 84 (1996).

\bibitem{mufun}
A.~{Gould}, {\it et~al.\/}, {Frequency of Solar-like Systems and of Ice and Gas
  Giants Beyond the Snow Line from High-magnification Microlensing Events in
  2005-2008}. {\it Astrophysical Journal\/} {\bf 720}, 1073 (2010).

\bibitem{Rhie00}
S.~H. {Rhie}, {\it et~al.\/}, {On Planetary Companions to the MACHO 98-BLG-35
  Microlens Star}. {\it Astrophysical Journal\/} {\bf 533}, 378 (2000).

\bibitem{Fernandes19}
R.~B. {Fernandes}, G.~D. {Mulders}, I.~{Pascucci}, C.~{Mordasini},
  A.~{Emsenhuber}, {Hints for a Turnover at the Snow Line in the Giant Planet
  Occurrence Rate}. {\it Astrophysical Journal\/} {\bf 874}, 81 (2019).

\bibitem{Bennett21}
D.~P. {Bennett}, C.~{Ranc}, R.~B. {Fernandes}, {No Sub-Saturn-mass Planet
  Desert in the CORALIE/HARPS Radial-velocity Sample}. {\it Astronomical Journal\/} {\bf 162},
  243 (2021).
  
\bibitem{Pass23}
E.~K. {Pass}, {\it et~al.\/}, {Mid-to-late M Dwarfs Lack Jupiter Analogs}. {\it
  Astronomical Journal\/} {\bf 166}, 11 (2023).

%%% Supplementary Materials Figure Captions %%%

%%% Supplementary Materials Table Captions %%%

\bibitem{OB190960}
J.~C. {Yee}, {\it et~al.\/}, {OGLE-2019-BLG-0960 Lb: the Smallest Microlensing
  Planet}. {\it Astronomical Journal\/} {\bf 162}, 180 (2021).

\bibitem{KB180029}
A.~{Gould}, {\it et~al.\/}, {KMT-2018-BLG-0029Lb: A Very Low Mass-Ratio Spitzer
  Microlens Planet}. {\it Journal of Korean Astronomical Society\/} {\bf 53}, 9
  (2020).

\bibitem{KB190842}
Y.~K. {Jung}, {\it et~al.\/}, {KMT-2019-BLG-0842Lb: A Cold Planet below the
  Uranus/Sun Mass Ratio}. {\it Astronomical Journal\/} {\bf 160}, 255 (2020).

\bibitem{OB161195}
Y.~{Shvartzvald}, {\it et~al.\/}, {An Earth-mass Planet in a 1 au Orbit around
  an Ultracool Dwarf}. {\it Astrophysical Journal\/} {\bf 840}, L3 (2017).

\bibitem{OB161195_MOA}
I.~A. {Bond}, {\it et~al.\/}, {The lowest mass ratio planetary microlens: OGLE
  2016-BLG-1195Lb}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 469}, 2434 (2017).

\bibitem{OB161195_true}
A.~{Gould}, {\it et~al.\/}, {OGLE-2016-BLG-1195 AO: Lens, Companion to Lens or
  Source, or None of the Above?} {\it Astronomical Journal\/} {\bf 166}, 145 (2023).
  
\bibitem{OB181185}
I.~{Kondo}, {\it et~al.\/}, {OGLE-2018-BLG-1185b: A Low-mass Microlensing
  Planet Orbiting a Low-mass Dwarf}. {\it Astronomical Journal\/} {\bf 162}, 77 (2021).

\bibitem{OB180383}
H.~{Wang}, {\it et~al.\/}, {Systematic Korea Microlensing Telescope Network
  planetary anomaly search - III. One wide-orbit planet and two stellar
  binaries}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 510}, 1778 (2022).

\bibitem{OB181269}
Y.~K. {Jung}, {\it et~al.\/}, {OGLE-2018-BLG-1269Lb: A Jovian Planet with a
  Bright I = 16 Host}. {\it Astronomical Journal\/} {\bf 160}, 148 (2020).

\bibitem{OB180567}
Y.~K. {Jung}, {\it et~al.\/}, {OGLE-2018-BLG-0567Lb and OGLE-2018-BLG-0962Lb:
  Two Microlensing Planets through the Planetary-caustic Channel}. {\it Astronomical Journal\/}
  {\bf 161}, 293 (2021).

\bibitem{Han2021three}
C.~{Han}, {\it et~al.\/}, {Three microlensing planets with no caustic-crossing
  features}. {\it Astronomy and Astrophysics\/} {\bf 650}, A89 (2021).

\bibitem{OB181428}
Y.~H. {Kim}, {\it et~al.\/}, {OGLE-2018-BLG-1428Lb: a Jupiter-mass planet
  beyond the snow line of a dwarf star}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 503}, 2706 (2021).

\bibitem{KB180748}
C.~{Han}, {\it et~al.\/}, {KMT-2018-BLG-0748Lb: sub-Saturn microlensing planet
  orbiting an ultracool host}. {\it Astronomy and Astrophysics\/} {\bf 641}, A105 (2020).

\bibitem{OB180799}
W.~{Zang}, {\it et~al.\/}, {OGLE-2018-BLG-0799Lb: a q 2.7 {\texttimes}
  10$^{-3}$ planet with Spitzer parallax}. {\it Mon. Not. R. Astron. Soc.\/} {\bf 514}, 5952
  (2022).

\bibitem{Chung23_ob1180}
S.-J. {Chung}, {\it et~al.\/}, {OGLE-2019-BLG-1180Lb: Discovery of a Wide-orbit
  Jupiter-mass Planet around a Late-type Star}. {\it Astronomical Journal\/} {\bf 166}, 253
  (2023).

\bibitem{KB181292}
Y.-H. {Ryu}, {\it et~al.\/}, {KMT-2018-BLG-1292: A Super-Jovian Microlens
  Planet in the Galactic Plane}. {\it Astronomical Journal\/} {\bf 159}, 58 (2020).

\bibitem{OB190468}
C.~{Han}, {\it et~al.\/}, {OGLE-2019-BLG-0468Lb,c: Two microlensing giant
  planets around a G-type star}. {\it Astronomy and Astrophysics\/} {\bf 658}, A93 (2022).

\bibitem{KB181990}
Y.-H. {Ryu}, {\it et~al.\/}, {KMT-2018-BLG-1990Lb: A Nearby Jovian Planet From
  A Low-cadence Microlensing Field}. {\it Astronomical Journal\/} {\bf 158}, 151 (2019).

\bibitem{OB180740}
C.~{Han}, {\it et~al.\/}, {Spectroscopic Mass and Host-star Metallicity
  Measurements for Newly Discovered Microlensing Planet OGLE-2018-BLG-0740Lb}.
  {\it Astronomical Journal\/} {\bf 158}, 102 (2019).

\bibitem{OB190362}
S.-J. {Chung}, {\it et~al.\/}, {OGLE-2019-BLG-0362Lb: A Super-Jovian-Mass
  Planet around a Low-Mass Star}. {\it Journal of Korean Astronomical
  Society\/} {\bf 55}, 123 (2022).

\bibitem{OB181011}
C.~{Han}, {\it et~al.\/}, {OGLE-2018-BLG-1011Lb,c: Microlensing Planetary
  System with Two Giant Planets Orbiting a Low-mass Star}. {\it Astronomical Journal\/} {\bf
  158}, 114 (2019).
  
\bibitem{Han2021resonant}
C.~{Han}, {\it et~al.\/}, {Three faint-source microlensing planets detected via
  the resonant-caustic channel}. {\it Astronomy and Astrophysics\/} {\bf 655}, A21 (2021).

\end{thebibliography}
